Multi-Agent Combinatorial-Multi-Armed-Bandit framework for the Submodular Welfare Problem under Bandit Feedback

We study the \emph{Submodular Welfare Problem} (SWP), where items are partitioned among agents with monotone submodular utilities to maximize the total welfare under \emph{bandit feedback}. Classical SWP assumes full value-oracle access, achieving $(1-1/e)$ approximations via continuous-greedy algorithms. We extend this to a \emph{multi-agent combinatorial bandit} framework (\textsc{MA-CMAB}), where actions are partitions under full-bandit feedback with non-communicating agents. Unlike prior single-agent or separable multi-agent CMAB models, our setting couples agents through shared allocation constraints. We propose an explore-then-commit strategy with randomized assignments, achieving $\tilde{\mathcal{O}}(T^{2/3})$ regret against a $(1-1/e)$ benchmark, the first such guarantee for partition-based submodular welfare problem under bandit feedback.

==> macro.tex <==


\usepackage{algorithm}
%\usepackage{algorithmic}

\usepackage{amsfonts}

% \usepackage{subcaption}
% \usepackage{algorithmic}
%\usepackage{algpseudocode}
% \newtheorem{sublemma}{Lemma}[lemma]
% \usepackage{amsmath}
% Recommended, but optional, packages for figures and better typesetting:
\usepackage{microtype}
\usepackage{graphicx}
% \usepackage{subfigure}
\usepackage{booktabs} % for professional tables

% hyperref makes hyperlinks in the resulting PDF.
% If your build breaks (sometimes temporarily if a hyperlink spans a page)
% please comment out the following usepackage line and replace
% \usepackage{icml2024} with \usepackage[nohyperref]{icml2024} above.
\usepackage{hyperref}


% Attempt to make hyperref and algorithmic work together better:


% Use the following line for the initial blind version submitted for review:
% \usepackage{icml2024}

% If accepted, instead use the following line for the camera-ready submission:


% For theorems and such
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{amsthm}
% if you use cleveref..
\usepackage[capitalize,noabbrev]{cleveref}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}


\usepackage{xcolor}
\usepackage{soul}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% THEOREMS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\theoremstyle{definition}
\newtheorem{definition}{Definition}
\newtheorem{assumption}{Assumption}
\theoremstyle*{remark}
\newtheorem*{remark}{Remark}[section]

% Todonotes is useful during development; simply uncomment the next line
%    and comment out the line below the next line to turn off comments
%\usepackage[disable,textsize=tiny]{todonotes}
\usepackage[textsize=footnotesize,color=orange!20]{todonotes}

%editing
\newcommand{\cjq}[1]{{\color{blue}#1}}
\newcommand{\shw}[1]{{\color{purple}#1}}


\newcommand{\blue}{\color{blue}}
\newcommand{\black}{\color{black}}
\newcommand{\gray}{\color{gray}}

\newcommand{\BCCMAB}{\text{BC-CMAB}}



%%%  Comment flags
\def\discussionSCalgchallenges{0}
    %there is a discussion in main section; notes in proof (added while CJQ was going over) rough, removing but if have time can polish















%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\usepackage[ruled, vlined]{algorithm2e}
\usepackage{amsmath}
\usepackage{mathtools}
\usepackage{enumitem}
\usepackage{thm-restate}
\usepackage{amsfonts}
\usepackage{mathtools}
\usepackage{tcolorbox}
\usepackage{amsthm}
\usepackage{xcolor}
\usepackage{graphicx} 
\usepackage{algorithmic}
\newcount\Comments  % 0 suppresses notes to selves in text
% \Comments=0
% \newcommand{\Comments}{1}
 % Enable comments
\newcommand{\kibitz}[2]{\ifnum\Comments=1{\textcolor{#1}{{#2}}}\fi}

\newcommand\tocite{\red{[CITE]}}
\newcommand\tocitec[1]{\red{[CITE: {#1}]}}
\definecolor{darkgreen}{rgb}{0,0.6,0}
\if 0
\newcommand{\kibitz}[2]{\ifnum\Comments=1{\textcolor{#1}{{#2}}}\fi}
\newcommand{\gan}[1]{\kibitz{blue}{[GG:#1]}}
\newcommand{\shw}[1]{\kibitz{red}{[SJ:#1]}}
\fi 


\newcommand{\van}[1]{\kibitz{purple}{[VA:#1]}}
\newcommand{\sub}[1]{\kibitz{orange}{[S:#1]}}
	    \newcommand{\red}[1]{{\leavevmode\color{red}{#1}}}
% \newcommand{\blue}[1]{{\leavevmode\color{blue}{#1}}}
\newcommand{\green}[1]{{\leavevmode\color[RGB]{0,128,0}{#1}}}
\newcommand{\purple}[1]{{\leavevmode\color[RGB]{128,0,255}{#1}}}
\newcommand{\orange}[1]{{\leavevmode\color[RGB]{229,83,0}{#1}}}
\newcommand{\lblue}[1]{{\leavevmode\color[RGB]{0,128,255}{#1}}}
\newcommand{\darkgray}[1]{{\leavevmode\color[RGB]{140,140,140}{#1}}}
\newcommand\TODO[1]{{\red{TODO: {#1}}}}


% \newcommand\tocite{\red{[CITE]}}

% \newcommand\tocitec[1]{\red{[CITE: {#1}]}}


\newcommand\toref{\red{[REF]}}
\newcommand\torefc[1]{\red{[REF: {#1}]}}
% \newtheorem{proposition}{Proposition}
% \newtheorem{lemma}{Lemma}
\newtheorem{observation}{Observation}
% \newtheorem{remark}{Remark}
\newcommand{\fairFrac}{\lceil \eta_H H \rceil}
\newcommand{\MINTSS}{\texttt{MINTSS}}

==> off_app_2.tex <==
\subsection{Bi-criteria Social welfare welfare with EF1 for additive valuation}
\begin{theorem}[\textsc{$\beta$-Majorization} Resilience]
\label{thm:CG:robust}
Under inexact utility evaluations \(|\hat{w}(S) - w(S)| \leq \epsilon\), for $\epsilon \le \omega\frac{c_{\min}}{4 n  c_{\max}}$, \textsc{continuous greedy} is an \((\alpha, \beta, \delta, \texttt{N})\)-resilient approximation algorithm for the Social Welfare with EF-1 (discrete partition) problem, where:
\[
\alpha = 1,\quad \beta=\frac{1}{2}, \quad 
%\delta = 6\frac{{c_{\max}}^2n^2}{c_{\min}}+2 \frac{n c_{\max}}{\omega}, \quad 
\delta = , \quad
\texttt{N} = NM^3,
\]
with \(c_{\max} = \max_{x \in \Omega} c_x\), \(c_{\min} = \min_{x \in \Omega} c_x\), and \(N = |\Omega|\).
\end{theorem}



We begin by quantifying how the total social welfare deviates under noisy oracle access.

\begin{lemma}[Resilience under Noisy Oracles]
\label{lemma:resilience}
Let each agent \( i \) have access to a noisy value oracle \( \hat{w}_i \) such that for any set \( S \subseteq \mathcal{X} \),
\[
|\hat{w}_i(S) - w_i(S)| \le \varepsilon.
\]
Suppose the allocation \( (S_1, \ldots, S_M) \) is obtained by sorting an EF1 partition constructed with respect to \( \hat{w}_i \), and let \( (S_1^*, \ldots, S_M^*) \) be the optimal EF1-constrained allocation under the true additive valuations \( w_i \). Then the expected social welfare satisfies:
\[
\sum_{i=1}^M w_i(S_i) \ge \frac{1}{2} \sum_{i=1}^M w_i(S_i^*) - \delta \varepsilon,
\]
where \( \delta = \frac{1}{2} \sum_{i=1}^n v_i + M \), and \( v_i \) are the (possibly normalized) agent bids.
\end{lemma}

\begin{proof}
From the noisy oracle guarantee, we have for any \( i \):
\[
w_i(S_i) \ge \hat{w}_i(S_i) - \varepsilon.
\]
Summing over all agents:
\[
\sum_{i=1}^M w_i(S_i) \ge \sum_{i=1}^M \hat{w}_i(S_i) - M\varepsilon. \tag{1}
\]

By Lemma~1 (majorization under EF1), sorting the EF1 partition based on \( \hat{w}_i \) ensures:
\[
\sum_{i=1}^M v_i \hat{w}_i(S_i) \ge \frac{1}{2} \sum_{i=1}^M v_i \hat{w}_i(S_i^*). \tag{2}
\]

Since \( \hat{w}_i(S_i^*) \ge w_i(S_i^*) - \varepsilon \), we get:
\[
\sum_{i=1}^M v_i \hat{w}_i(S_i^*) \ge \sum_{i=1}^M v_i w_i(S_i^*) - \varepsilon \sum_{i=1}^M v_i. \tag{3}
\]

Substituting (3) into (2), and then into (1):
\[
\sum_{i=1}^M w_i(S_i) \ge \frac{1}{2} \sum_{i=1}^M v_i w_i(S_i^*) - \left( \frac{1}{2} \sum_{i=1}^M v_i + M \right) \varepsilon,
\]
as claimed.
\end{proof}
\begin{remark}
    From Lipton cite{} proposed poly time oracle call based algorithm is $NM^3$ just guarantee EF-1 through cycle elimination further $\frac{1}{2}$ USW is commaon to achieve for any additive valuation function  where partition is any EF-1 
 partition case mentioned in Sidharth \cite{sid}.
\end{remark}
\vspace{0.5em}

\subsection{Stability of EF1 Guarantee under Noisy Valuations}

We now show that an EF1 allocation computed with respect to noisy oracle access remains approximately EF1 with respect to true valuations.

\begin{lemma}[Approximate EF1 under Noisy Oracles]
\label{lemma:ef1-noise}
Let \( S = (S_1, \ldots, S_M) \) be an allocation that satisfies the EF1 condition with respect to noisy value oracles \( \hat{w}_i \), where
\[
|\hat{w}_i(S) - w_i(S)| \le \varepsilon \quad \text{for all } i, S.
\]
Then for every pair of agents \( i, j \in [M] \), there exists a good \( g \in S_j \) such that:
\[
w_i(S_i) \ge w_i(S_j \setminus \{g\}) - 2\varepsilon.
\]
\end{lemma}

\begin{proof}
By EF1 under the noisy oracle, for every pair \( (i, j) \), there exists \( g \in S_j \) such that:
\[
\hat{w}_i(S_i) \ge \hat{w}_i(S_j \setminus \{g\}).
\]

Using the oracle error bounds:
\[
w_i(S_i) \ge \hat{w}_i(S_i) - \varepsilon, \quad \text{and} \quad w_i(S_j \setminus \{g\}) \le \hat{w}_i(S_j \setminus \{g\}) + \varepsilon.
\]

Then:
\[
w_i(S_i) \ge \hat{w}_i(S_j \setminus \{g\}) - \varepsilon \ge w_i(S_j \setminus \{g\}) - 2\varepsilon,
\]
which proves that the EF1 guarantee is preserved up to an additive slack of \( 2\varepsilon \).
\end{proof}

